Navigating the Effect of Parametrization for Dimensionality Reduction

Parametric dimensionality reduction methods have gained prominence for their ability to generalize to unseen datasets, an advantage that traditional approaches typically lack. Despite their growing popularity, there remains a prevalent misconception among practitioners about the equivalence in performance between parametric and non-parametric methods. Here, we show that these methods are not equivalent -- parametric methods retain global structure but lose significant local details. To explain this, we provide evidence that parameterized approaches lack the ability to repulse negative pairs, and the choice of loss function also has an impact. Addressing these issues, we developed a new parametric method, ParamRepulsor, that incorporates Hard Negative Mining and a loss function that applies a strong repulsive force. This new method achieves state-of-the-art performance on local structure preservation for parametric methods without sacrificing the fidelity of global structural representation. Our code is available at https://github.com/hyhuang00/ParamRepulsor.

==> figures/scripts/fig_arch_comp.tex <==

\begin{figure}[tbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/figures/fig_comp_arch.png}
        \caption{Behavior of Parametric DR algorithms under different learning rate (lr), architecture, and batch size (bsz).}
        \label{fig:comp_arch}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/figures/fig_paramchange.png}
        \caption{Change.}
        \label{fig:paramch}
    \end{subfigure}
    \caption{}
    \label{fig: dilation}
\vspace{-0.1in}
\end{figure}


==> figures/scripts/localstructure.tex <==
\begin{figure*}[tbh]
\includegraphics[width=\textwidth]{figures/figures/fig_localgeneral.png}

\vspace{-0.15in}

\caption{SVM and 10-NN Accuracy measured on various datasets. Missing bars suggest method unable to process a dataset.}
\label{fig:localst}
\end{figure*}


==> figures/scripts/lossratio.tex <==
\begin{figure*}[th]
\includegraphics[width=\textwidth]{figures/figures/fig_loss_box.png}
\vspace{-0.3in}

\caption{Loss of the ParamPaCMAP embedding compared to original ParamPaCMAP on non-generated datasets.}
\label{fig:lossratio}
\end{figure*}


==> figures/scripts/mammoth.tex <==
\begin{figure*}[ht]
\includegraphics[width=0.9\textwidth]{figures/figures/fig_mammoth_2.png}
\vspace{-0.2in}
\caption{Dimensionality Reduction results of the Mammoth dataset by various DR methods \cite{SmithsonianMammoth}. Classical nonparametric methods failed to preserve the global structure of the mammoth.}
\label{fig:mammothintro}
\vspace{-0.22in}
\end{figure*}


==> parampacmap_impl.tex <==
\section{Implementation details for Baseline Parametric PaCMAP}
\label{sec:parampacmap}
In order to faithfully reflect the impact of parametrization on the embedding, our baseline parametric pacmap 

\paragraph{Network Structure.} In line with existing parametric DR method implementation \cite{sainburg2021parametric, damrich2023from}, we parametrize the projector with a shallow Multi-layer Perceptron. Unless otherwise specified, we utilize a network of three hidden layers with [100, 100, 100] neurons. We also use ReLU as our activation function for the baseline implementation.

\paragraph{Initialization.} As a non-parametric algorithm, PaCMAP directly optimizes the low-dimensional embedding, and utilizes the first two principal components of the data as its initialization. After the introduction of the neural network projector, we can no longer use this initialization. We initialize all our neural network parameters with Kaiming Initialization \cite{he2016deep}.

\paragraph{Optimization Schedule.}
Since our neural network optimization schedule is performed by mini-batch stochastic gradient descent, we are unable to optimize the full embedding at once as in non-parametric PaCMAP. Therefore, at each step, we sample a batch of points, and find NN, MN, and FP pairs for each element in the sample. All the points will be sent to the neural network to calculate the standard PaCMAP loss. We adopt the Adam Optimizer \cite{kingma2014adam} with $\beta=(0.9, 0.999)$ and a batch size of 1024.

